Real-time Inflation Forecasting Using Non-linear Dimension Reduction Techniques

In this paper, we assess whether using non-linear dimension reduction techniques pays off for forecasting inflation in real-time. Several recent methods from the machine learning literature are adopted to map a large dimensional dataset into a lower dimensional set of latent factors. We model the relationship between inflation and the latent factors using constant and time-varying parameter (TVP) regressions with shrinkage priors. Our models are then used to forecast monthly US inflation in real-time. The results suggest that sophisticated dimension reduction methods yield inflation forecasts that are highly competitive to linear approaches based on principal components. Among the techniques considered, the Autoencoder and squared principal components yield factors that have high predictive power for one-month- and one-quarter-ahead inflation. Zooming into model performance over time reveals that controlling for non-linear relations in the data is of particular importance during recessionary episodes of the business cycle or the current COVID-19 pandemic.

==> final_rmse_lps_approx_2019.917_main_1.tex <==
%latex.default(final.tab.1, file = paste0(tab.dir, "/", vint,     "_", type, "_", lps_type, "_", eval.prds[length(eval.prds)],     "_", var.type, "_1.tex"), title = "", ctable = FALSE, rgroupTexCmd = "scshape",     rownamesTexCmd = my.rownamesTexCmd, n.cgroup = n.cgroup,     cgroup = cgroup.1, colheads = colheads, rgroup = rgroup,     n.rgroup = n.rgroup, caption = "", label = "tab:LPS", size = "tiny",     booktabs = TRUE, rowname = "", numeric.dollar = FALSE, caption.loc = "bottom",     landscape = FALSE)%
\begin{table*}[!tbp]
{\tiny
\begin{center}
\caption{One-month-ahead forecast performance. \label{tab:main1}}
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} llcllll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{1}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{4}{c}{\bfseries One-month ahead}\tabularnewline
\cline{2-2} \cline{4-7}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{const. (MIN)}&\multicolumn{1}{c}{const. (HS)}&\multicolumn{1}{c}{TVP std. (MIN)}&\multicolumn{1}{c}{TVP std. (HS)}\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
\shadeBench   ~~&   AR&   &   -300.16&    -2.99&   -2.29&    -4.20\tabularnewline
\shadeBench   ~~&   &   &   (1.15)&   (0.99)&   (0.98)&   (0.99)\tabularnewline
   ~~&   Large PC&   &     -1.93&   -10.67***&      &   \textbf{-9.74***}\tabularnewline
   ~~&   &   &   (0.98)&   (1.06***)&   &   (\textbf{1.04***})\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   Autoencoder 1l (k = 05)&   &     -0.64&    -4.18&   -1.43&    -3.94\tabularnewline
   ~~&   &   &   (0.98)&   (0.99)&   (0.98)&   (0.99)\tabularnewline
   ~~&   Autoencoder 1l (k = 15)&   &     11.43***&     9.35**&   15.92***&     9.81**\tabularnewline
   ~~&   &   &   (0.90**)&   (0.91**)&   (0.87***)&   (0.91**)\tabularnewline
   ~~&   Autoencoder 1l (k = 30)&   &   \textbf{23.93***}&   \textbf{20.25***}&   21.45**&   \textbf{20.66***}\tabularnewline
   ~~&   &   &   (\textbf{0.84***})&   (\textbf{0.86***})&   (\textbf{0.83***})&   (\textbf{0.85***})\tabularnewline
   ~~&   Autoencoder 3l (k = 05)&   &      0.03&    -4.10&   -1.42&    -4.73\tabularnewline
   ~~&   &   &   (0.98)&   (0.99)&   (0.97)&   (0.99)\tabularnewline
   ~~&   Autoencoder 3l (k = 15)&   &      5.15&     3.41&    7.86&     3.86\tabularnewline
   ~~&   &   &   (0.95)&   (0.96)&   (0.93*)&   (0.95)\tabularnewline
   ~~&   Autoencoder 3l (k = 30)&   &     19.38***&    16.78***&   14.85&    14.05**\tabularnewline
   ~~&   &   &   (0.86***)&   (0.88***)&   (0.84***)&   (0.87***)\tabularnewline
   ~~&   Autoencoder 5l (k = 05)&   &     -0.90&    -4.68&   -1.71&    -5.36\tabularnewline
   ~~&   &   &   (0.98)&   (0.99)&   (0.98)&   (0.99)\tabularnewline
   ~~&   Autoencoder 5l (k = 15)&   &      5.29&     2.01&    6.19&     3.89\tabularnewline
   ~~&   &   &   (0.95)&   (0.95)&   (0.94)&   (0.94)\tabularnewline
   ~~&   Autoencoder 5l (k = 30)&   &     21.90***&    20.00***&   \textbf{21.67**}&    20.62***\tabularnewline
   ~~&   &   &   (0.85***)&   (0.86***)&   (0.85***)&   (0.86***)\tabularnewline
   ~~&   Autoencoder 8l (k = 05)&   &     -1.23&    -4.77&    1.00&    -5.00\tabularnewline
   ~~&   &   &   (0.98)&   (1.00)&   (0.98)&   (0.99)\tabularnewline
   ~~&   Autoencoder 8l (k = 15)&   &     -1.06&    -6.10**&   -1.84&    -4.41\tabularnewline
   ~~&   &   &   (0.98)&   (1.01)&   (0.98)&   (1.00)\tabularnewline
   ~~&   Autoencoder 8l (k = 30)&   &      1.37&    -2.21&    3.31&    -2.33\tabularnewline
   ~~&   &   &   (0.97)&   (0.99)&   (0.96)&   (0.98)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   Diffusion Maps (k = 05)&   &     -0.44&    -5.38&    0.01&    -4.13\tabularnewline
   ~~&   &   &   (0.99)&   (1.01)&   (0.98)&   (1.01)\tabularnewline
   ~~&   Diffusion Maps (k = 15)&   &     -0.74&    -9.97***&   -0.53&    -9.11***\tabularnewline
   ~~&   &   &   (0.99)&   (1.03***)&   (0.99)&   (1.03**)\tabularnewline
   ~~&   Diffusion Maps (k = 30)&   &     -0.33&   -10.93***&    0.78&    -8.68***\tabularnewline
   ~~&   &   &   (0.98)&   (1.03***)&   (0.98)&   (1.02**)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   ISOMAP (k = 05)&   &     -0.64&    -5.23&   -0.03&    -3.84\tabularnewline
   ~~&   &   &   (0.98)&   (0.99)&   (0.98)&   (0.99)\tabularnewline
   ~~&   ISOMAP (k = 15)&   &      0.18&    -6.35**&   -1.60&    -6.00**\tabularnewline
   ~~&   &   &   (0.98)&   (1.01)&   (0.98)&   (1.01)\tabularnewline
   ~~&   ISOMAP (k = 30)&   &     -1.32&    -6.20***&    0.05&    -5.62**\tabularnewline
   ~~&   &   &   (0.98)&   (1.01**)&   (0.98)&   (1.01)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   LLE (k = 05)&   &     -1.49&    -4.20&   -0.88&    -4.05\tabularnewline
   ~~&   &   &   (0.98)&   (1.00)&   (0.99)&   (1.00)\tabularnewline
   ~~&   LLE (k = 15)&   &     -0.20&    -6.66***&   -1.33&    -5.78**\tabularnewline
   ~~&   &   &   (0.98)&   (1.02*)&   (0.98)&   (1.01)\tabularnewline
   ~~&   LLE (k = 30)&   &     -0.97&   -10.18*&   -1.79&   -10.72**\tabularnewline
   ~~&   &   &   (0.98)&   (1.01)&   (0.98)&   (1.00)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   PCA gauss. kernel (k = 05)&   &     -0.69&    -4.23&   -0.92&    -2.86\tabularnewline
   ~~&   &   &   (0.98)&   (1.00)&   (0.98)&   (0.99)\tabularnewline
   ~~&   PCA gauss. kernel (k = 15)&   &     -0.83&    -4.09&   -1.00&    -5.64\tabularnewline
   ~~&   &   &   (0.99)&   (1.00)&   (0.98)&   (1.00)\tabularnewline
   ~~&   PCA gauss. kernel (k = 30)&   &     -0.63&    -4.84&    0.58&    -3.29\tabularnewline
   ~~&   &   &   (0.98)&   (1.00)&   (0.98)&   (0.99)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   PCA linear (k = 05)&   &     -0.85&    -6.05&   -1.38&    -5.13\tabularnewline
   ~~&   &   &   (0.98)&   (1.01)&   (0.99)&   (1.00)\tabularnewline
   ~~&   PCA linear (k = 15)&   &      0.81&    -6.25**&    0.51&    -5.86*\tabularnewline
   ~~&   &   &   (0.98)&   (1.01)&   (0.98)&   (1.00)\tabularnewline
   ~~&   PCA linear (k = 30)&   &      0.05&    -8.09***&   -1.12&    -7.16**\tabularnewline
   ~~&   &   &   (0.98)&   (1.02**)&   (0.98)&   (1.02*)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   PCA poly. kernel (k = 05)&   &      0.30&    -3.77&   -0.43&    -2.95\tabularnewline
   ~~&   &   &   (0.99)&   (1.00)&   (0.98)&   (0.99)\tabularnewline
   ~~&   PCA poly. kernel (k = 15)&   &     -1.57&    -3.34&   -0.34&    -4.87\tabularnewline
   ~~&   &   &   (0.98)&   (0.99)&   (0.98)&   (0.99)\tabularnewline
   ~~&   PCA poly. kernel (k = 30)&   &     -0.05&    -5.60&   -1.22&    -5.16\tabularnewline
   ~~&   &   &   (0.98)&   (1.00)&   (0.98)&   (1.00)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   PCA quadratic (k = 05)&   &      6.05&     2.92&    5.22&     3.18\tabularnewline
   ~~&   &   &   (0.91)&   (0.94)&   (0.90)&   (0.93)\tabularnewline
   ~~&   PCA quadratic (k = 15)&   &      0.56&    -3.45&    2.32&    -2.21\tabularnewline
   ~~&   &   &   (1.01)&   (0.99)&   (0.98)&   (0.98)\tabularnewline
   ~~&   PCA quadratic (k = 30)&   &     -0.99&    -8.79**&    2.93&    -6.38\tabularnewline
   ~~&   &   &   (0.98)&   (1.04**)&   (0.96)&   (1.03**)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   PCA squared (k = 05)&   &      5.18&     3.53&    6.23&     2.70\tabularnewline
   ~~&   &   &   (0.90)&   (0.93)&   (0.89)&   (0.92)\tabularnewline
   ~~&   PCA squared (k = 15)&   &      1.65&    -3.32&    2.73&    -2.14\tabularnewline
   ~~&   &   &   (0.98)&   (0.98)&   (0.93)&   (0.98)\tabularnewline
   ~~&   PCA squared (k = 30)&   &      0.34&    -2.97&    4.47&    -5.81\tabularnewline
   ~~&   &   &   (0.98)&   (1.02*)&   (0.95)&   (1.02*)\tabularnewline
\bottomrule
\end{tabular*}
\begin{tablenotes}[flushleft]
\tiny
\item \textit{Note:} The table shows LPLs with RMSEs in parentheses below. The first (red shaded) entry gives the actual LPL and RMSE scores of our benchmark (an autoregressive (AR) model with constant parameters and a Minnesota prior). Asterisks indicate statistical significance for each model relative to the benchmark at the 1\% (***), 5\% (**) and 10\% (*) significance levels. Since the large ARX model with time-varying parameters would features $273$ period-specific coefficients and is computationally intractable, we assume that the TVPs feature a factor structure (with three factors) to reduce the dimension of the state space \citep[see Section \ref{sec:App B} of the Online Appendix and][]{chan2020reducing}. 
\end{tablenotes}
\end{center}}
\end{table*}


==> final_rmse_lps_approx_2019.917_main_3.tex <==
%latex.default(final.tab.312, file = paste0(tab.dir, "/", vint,     "_", type, "_", lps_type, "_", eval.prds[length(eval.prds)],     "_", var.type, "_3.tex"), title = "", ctable = FALSE, rgroupTexCmd = "scshape",     rownamesTexCmd = my.rownamesTexCmd, n.cgroup = n.cgroup,     cgroup = cgroup.3, colheads = colheads, rgroup = rgroup,     n.rgroup = n.rgroup, caption = "", label = "tab:LPS", size = "tiny",     booktabs = TRUE, rowname = "", numeric.dollar = FALSE, caption.loc = "bottom",     landscape = FALSE)%
\begin{table*}[!tbp]
{\tiny
\begin{center}
\caption{One-quarter-ahead forecast performance. \label{tab:main3}}
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} llcllll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{1}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{4}{c}{\bfseries One-quarter ahead}\tabularnewline
\cline{2-2} \cline{4-7}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{const. (MIN)}&\multicolumn{1}{c}{const. (HS)}&\multicolumn{1}{c}{TVP std. (MIN)}&\multicolumn{1}{c}{TVP std. (HS)}\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
\shadeBench   ~~&   AR&   &   -306.39&    10.04&    12.04&    10.37\tabularnewline
\shadeBench   ~~&   &   &   (1.21)&   (0.94*)&   (0.90)&   (0.90)\tabularnewline
   ~~&   Large PC&   &     -2.71&    -3.74&       &   \textbf{-8.72}\tabularnewline
   ~~&   &   &   (0.92)&   (0.98)&   &   (\textbf{0.99})\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   Autoencoder 1l (k = 05)&   &     -0.32&   -10.11&    -4.29&    -8.79\tabularnewline
   ~~&   &   &   (0.92)&   (0.93)&   (0.93)&   (0.93)\tabularnewline
   ~~&   Autoencoder 1l (k = 15)&   &      4.58&     0.13&     2.40&     0.17\tabularnewline
   ~~&   &   &   (0.89)&   (0.90)&   (0.90)&   (0.90)\tabularnewline
   ~~&   Autoencoder 1l (k = 30)&   &      3.97&     4.69&     5.94&     4.09\tabularnewline
   ~~&   &   &   (0.88)&   (0.88)&   (0.88)&   (0.88)\tabularnewline
   ~~&   Autoencoder 3l (k = 05)&   &     -0.80&    -4.79&     1.62&    -6.61\tabularnewline
   ~~&   &   &   (0.90)&   (0.90)&   (0.90)&   (0.90)\tabularnewline
   ~~&   Autoencoder 3l (k = 15)&   &      1.82&    -3.05&     1.30&    -5.21\tabularnewline
   ~~&   &   &   (0.89)&   (0.90)&   (0.90)&   (0.89)\tabularnewline
   ~~&   Autoencoder 3l (k = 30)&   &      4.53&    -6.02&     2.43&    -3.99\tabularnewline
   ~~&   &   &   (0.89)&   (0.89)&   (0.89)&   (0.89)\tabularnewline
   ~~&   Autoencoder 5l (k = 05)&   &      2.02&   -10.49&    -2.49&    -7.56\tabularnewline
   ~~&   &   &   (0.90)&   (0.90)&   (0.90)&   (0.90)\tabularnewline
   ~~&   Autoencoder 5l (k = 15)&   &     -1.07&   -10.96&    -1.76&    -9.55\tabularnewline
   ~~&   &   &   (0.89)&   (0.90)&   (0.89)&   (0.90)\tabularnewline
   ~~&   Autoencoder 5l (k = 30)&   &      3.37&    -3.35&     0.06&    -4.18\tabularnewline
   ~~&   &   &   (0.89)&   (0.89)&   (0.89)&   (0.88)\tabularnewline
   ~~&   Autoencoder 8l (k = 05)&   &      2.57&    -7.87&    -1.84&    -8.87\tabularnewline
   ~~&   &   &   (0.92)&   (0.93)&   (0.93)&   (0.94)\tabularnewline
   ~~&   Autoencoder 8l (k = 15)&   &    -10.28&   -21.52&   -13.30&   -21.51\tabularnewline
   ~~&   &   &   (0.92)&   (0.96)&   (0.93)&   (0.96)\tabularnewline
   ~~&   Autoencoder 8l (k = 30)&   &    -25.45&   -40.95*&   -33.35&   -41.72*\tabularnewline
   ~~&   &   &   (0.93)&   (0.95)&   (0.93)&   (0.95)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   Diffusion Maps (k = 05)&   &     -0.02&     2.12&    -2.35&    -1.25\tabularnewline
   ~~&   &   &   (0.89)&   (0.89)&   (0.89)&   (0.89)\tabularnewline
   ~~&   Diffusion Maps (k = 15)&   &      3.80&    -1.52&     1.56&    -3.16\tabularnewline
   ~~&   &   &   (0.90)&   (0.90)&   (0.89)&   (0.90)\tabularnewline
   ~~&   Diffusion Maps (k = 30)&   &     -1.18&    -7.01&     5.04&    -6.54\tabularnewline
   ~~&   &   &   (0.90)&   (0.92)&   (0.90)&   (0.92)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   ISOMAP (k = 05)&   &      1.16&    -3.74&    -0.71&    -2.95\tabularnewline
   ~~&   &   &   (0.89)&   (0.89)&   (0.90)&   (0.89)\tabularnewline
   ~~&   ISOMAP (k = 15)&   &      2.65&    -9.85&    -1.23&    -9.94\tabularnewline
   ~~&   &   &   (0.89)&   (0.90)&   (0.90)&   (0.90)\tabularnewline
   ~~&   ISOMAP (k = 30)&   &     -2.55&   -10.81&    -7.53&   -12.79\tabularnewline
   ~~&   &   &   (0.89)&   (0.89)&   (0.90)&   (0.89)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   LLE (k = 05)&   &     -1.81&   -11.86&    -7.79&   -11.78\tabularnewline
   ~~&   &   &   (0.90)&   (0.91)&   (0.90)&   (0.91)\tabularnewline
   ~~&   LLE (k = 15)&   &    -30.30&   -34.55&   -32.43&   -30.84\tabularnewline
   ~~&   &   &   (0.91)&   (0.93)&   (0.92)&   (0.92)\tabularnewline
   ~~&   LLE (k = 30)&   &    -17.24&   -52.70&   -26.06&   -52.63\tabularnewline
   ~~&   &   &   (0.91)&   (0.92)&   (0.92)&   (0.92)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   PCA gauss. kernel (k = 05)&   &     -1.32&    -6.67&     0.62&    -9.68\tabularnewline
   ~~&   &   &   (0.92)&   (0.92)&   (0.92)&   (0.93)\tabularnewline
   ~~&   PCA gauss. kernel (k = 15)&   &     -3.97&   -12.66&    -4.10&    -9.22\tabularnewline
   ~~&   &   &   (0.92)&   (0.93)&   (0.92)&   (0.93)\tabularnewline
   ~~&   PCA gauss. kernel (k = 30)&   &      0.26&    -7.47&    -1.28&    -7.36\tabularnewline
   ~~&   &   &   (0.91)&   (0.92)&   (0.91)&   (0.92)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   PCA linear (k = 05)&   &     -2.99&   -10.80&    -5.92&   -11.36\tabularnewline
   ~~&   &   &   (0.93)&   (0.95)&   (0.94)&   (0.95)\tabularnewline
   ~~&   PCA linear (k = 15)&   &     -2.95&    -7.21&    -6.30&   -12.38\tabularnewline
   ~~&   &   &   (0.92)&   (0.93)&   (0.93)&   (0.93)\tabularnewline
   ~~&   PCA linear (k = 30)&   &      1.55&    -6.30&    -0.10&    -5.63\tabularnewline
   ~~&   &   &   (0.91)&   (0.92)&   (0.91)&   (0.91)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   PCA poly. kernel (k = 05)&   &     -0.75&    -9.56&    -4.40&   -11.61\tabularnewline
   ~~&   &   &   (0.93)&   (0.94)&   (0.93)&   (0.94)\tabularnewline
   ~~&   PCA poly. kernel (k = 15)&   &     -2.16&    -8.26&    -2.40&    -6.52\tabularnewline
   ~~&   &   &   (0.92)&   (0.92)&   (0.92)&   (0.92)\tabularnewline
   ~~&   PCA poly. kernel (k = 30)&   &      2.09&    -4.45&    -0.07&    -2.96\tabularnewline
   ~~&   &   &   (0.91)&   (0.91)&   (0.91)&   (0.91)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   PCA quadratic (k = 05)&   &     16.59&   \textbf{22.51}&    17.55&    22.30\tabularnewline
   ~~&   &   &   (0.89)&   (0.84)&   (0.88)&   (0.84)\tabularnewline
   ~~&   PCA quadratic (k = 15)&   &     -5.54&     5.06&    -6.54&     6.52\tabularnewline
   ~~&   &   &   (0.96)&   (0.91)&   (0.95)&   (0.91)\tabularnewline
   ~~&   PCA quadratic (k = 30)&   &      4.75&    -0.04&     5.94&     1.62\tabularnewline
   ~~&   &   &   (0.91)&   (0.94)&   (0.91)&   (0.95)\tabularnewline
\midrule
{\scshape }&&&&&&\tabularnewline
   ~~&   PCA squared (k = 05)&   &   \textbf{23.05}&    22.36&   \textbf{22.58}&   \textbf{22.98}\tabularnewline
   ~~&   &   &   (\textbf{0.84})&   (\textbf{0.81})&   (\textbf{0.85})&   (\textbf{0.81})\tabularnewline
   ~~&   PCA squared (k = 15)&   &      0.74&     4.99&     0.89&     5.91\tabularnewline
   ~~&   &   &   (0.92)&   (0.92)&   (0.92)&   (0.93)\tabularnewline
   ~~&   PCA squared (k = 30)&   &      7.89&     3.38&     7.06&     2.16\tabularnewline
   ~~&   &   &   (0.90)&   (0.92)&   (0.90)&   (0.92)\tabularnewline
\bottomrule
\end{tabular*}
\begin{tablenotes}[flushleft]
\tiny
\item \textit{Note:} The table shows LPLs with RMSEs in parentheses below. The first (red shaded) entry gives the actual LPL and RMSE scores of our benchmark (an autoregressive (AR) model with constant parameters and a Minnesota prior). Asterisks indicate statistical significance for each model relative to the benchmark at the 1\% (***), 5\% (**) and 10\% (*) significance levels. Since the large ARX model with time-varying parameters would features $273$ period-specific coefficients and is computationally intractable, we assume that the TVPs feature a factor structure (with three factors) to reduce the dimension of the state space \citep[see Section \ref{sec:App B} of the Online Appendix and][]{chan2020reducing}. 
\end{tablenotes}
\end{center}}
\end{table*}


==> table_corr_var_AE.tex <==
%latex.default(final.tab, file = paste0(dir, "/scores/table_corr_var_AE.tex"),     title = "", ctable = FALSE, rgroupTexCmd = "scshape", rownamesTexCmd = my.rownamesTexCmd,     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     rgroup = rgroup, n.rgroup = n.rgroup, caption = "", label = "tab:LPS",     size = "tiny", booktabs = TRUE, rowname = "", numeric.dollar = FALSE,     caption.loc = "bottom", landscape = FALSE)%
\begin{table*}
{\tiny
\caption{Top-five correlated variables with each factor for the Autoencoder with 1 layer and 30 factors \label{tab:corr_ae}}
\begin{center}
\begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} lcccccccccc}
\toprule
\multicolumn{1}{l}{\bfseries }& \bfseries Seq. of factors &\multicolumn{10}{c}{\bfseries Top-5 correlated variables}\tabularnewline
\multicolumn{1}{l}{}& (Autoencoder 1l) &\multicolumn{1}{c}{}&\multicolumn{1}{c}{1}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{2}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{3}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{4}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{5}\tabularnewline
\midrule
   ~~&   Factor 1&   &   PERMITMW&   &   HOUSTMW&   &   T5YFFM&   &   CES0600000007&   &   PERMIT\tabularnewline
   ~~&   Factor 2&   &   PERMITS&   &   HOUSTS&   &   HOUST&   &   PERMIT&   &   PERMITW\tabularnewline
   ~~&   Factor 3&   &   HOUST&   &   PERMIT&   &   PERMITS&   &   HOUSTS&   &   HOUSTW\tabularnewline
   ~~&   Factor 4&   &   HOUSTS&   &   HOUST&   &   PERMIT&   &   PERMITW&   &   PERMITS\tabularnewline
   ~~&   Factor 5&   &   BAAFFM&   &   AAAFFM&   &   T10YFFM&   &   T5YFFM&   &   CES0600000007\tabularnewline
   ~~&   Factor 6&   &   PERMITS&   &   PERMITW&   &   HOUSTW&   &   PERMIT&   &   HOUST\tabularnewline
   ~~&   Factor 7&   &   CES0600000007&   &   AWHMAN&   &   CES1021000001&   &   HOUSTMW&   &   PERMITMW\tabularnewline
   ~~&   Factor 8&   &   CES0600000007&   &   AWHMAN&   &   HOUSTS&   &   PERMITS&   &   HOUST\tabularnewline
   ~~&   Factor 9&   &   AMDMUOx&   &   BAAFFM&   &   AAAFFM&   &   BUSINVx&   &   USWTRADE\tabularnewline
   ~~&   Factor 10&   &   AWHMAN&   &   CES0600000007&   &   PERMITMW&   &   HOUSTMW&   &   HOUST\tabularnewline
   ~~&   Factor 11&   &   PERMITMW&   &   HOUSTMW&   &   PERMIT&   &   HOUST&   &   T5YFFM\tabularnewline
   ~~&   Factor 12&   &   AWHMAN&   &   CES0600000007&   &   TB3SMFFM&   &   TB6SMFFM&   &   HOUSTMW\tabularnewline
   ~~&   Factor 13&   &   PERMITMW&   &   HOUSTMW&   &   HOUST&   &   PERMIT&   &   PERMITW\tabularnewline
   ~~&   Factor 14&   &   PERMITMW&   &   PERMIT&   &   HOUST&   &   PERMITW&   &   HOUSTW\tabularnewline
   ~~&   Factor 15&   &   PERMITMW&   &   HOUSTMW&   &   T5YFFM&   &   PERMIT&   &   HOUST\tabularnewline
   ~~&   Factor 16&   &   PERMITMW&   &   HOUSTMW&   &   HOUST&   &   PERMIT&   &   PERMITW\tabularnewline
   ~~&   Factor 17&   &   HOUST&   &   PERMIT&   &   PERMITS&   &   HOUSTS&   &   PERMITW\tabularnewline
   ~~&   Factor 18&   &   T1YFFM&   &   TB6SMFFM&   &   PERMITMW&   &   PERMITS&   &   PERMIT\tabularnewline
   ~~&   Factor 19&   &   FEDFUNDS&   &   TB6MS&   &   TB3MS&   &   CP3Mx&   &   GS1\tabularnewline
   ~~&   Factor 20&   &   CES0600000007&   &   HOUSTMW&   &   PERMITMW&   &   HOUST&   &   HOUSTS\tabularnewline
   ~~&   Factor 21&   &   PERMITS&   &   PERMITW&   &   PERMIT&   &   HOUSTS&   &   HOUSTW\tabularnewline
   ~~&   Factor 22&   &   CES0600000007&   &   AWHMAN&   &   T1YFFM&   &   TB6SMFFM&   &   T5YFFM\tabularnewline
   ~~&   Factor 23&   &   TB6SMFFM&   &   TB3SMFFM&   &   T1YFFM&   &   AWHMAN&   &   CES0600000007\tabularnewline
   ~~&   Factor 24&   &   FEDFUNDS&   &   TB6SMFFM&   &   TB6MS&   &   TB3MS&   &   CP3Mx\tabularnewline
   ~~&   Factor 25&   &   BAAFFM&   &   AAAFFM&   &   T10YFFM&   &   T5YFFM&   &   AMDMUOx\tabularnewline
   ~~&   Factor 26&   &   PERMITMW&   &   HOUSTMW&   &   HOUST&   &   PERMIT&   &   HOUSTW\tabularnewline
   ~~&   Factor 27&   &   PERMITMW&   &   HOUSTMW&   &   CES0600000007&   &   AWHMAN&   &   HOUST\tabularnewline
   ~~&   Factor 28&   &   PERMITW&   &   PERMITS&   &   PERMIT&   &   HOUSTS&   &   HOUST\tabularnewline
   ~~&   Factor 29&   &   FEDFUNDS&   &   TB3MS&   &   TB6MS&   &   BUSINVx&   &   CP3Mx\tabularnewline
   ~~&   Factor 30&   &   PERMITMW&   &   HOUSTMW&   &   HOUST&   &   PERMITNE&   &   HOUSTNE\tabularnewline
\bottomrule
\end{tabular*}
\begin{tablenotes}[flushleft]
      \tiny
      \item \textit{Note:} The table shows the first five variables with the highest correlation for each factor obtained from the Autoencoder specification with 1 layer and 30 factors.
    \end{tablenotes}
\end{center}}
\end{table*}

